PANORAMIA: Privacy Auditing of Machine Learning Models without Retraining

We present PANORAMIA, a privacy leakage measurement framework for machine learning models that relies on membership inference attacks using generated data as non-members. By relying on generated non-member data, PANORAMIA eliminates the common dependency of privacy measurement tools on in-distribution non-member data. As a result, PANORAMIA does not modify the model, training data, or training process, and only requires access to a subset of the training data. We evaluate PANORAMIA on ML models for image and tabular data classification, as well as on large-scale language models.

==> src/O1-comparisons.tex <==
\subsection{Target ML Model Trained on Real Data}
\begin{table} [t]
    \centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{Target model} & \textbf{Audit} & $\mathbf{c_{lb}}$ & $\mathbf{\varepsilon + c_{lb}}$ & $\mathbf{\tilde{\varepsilon}}$ & $\mathbf{\varepsilon}$ \\
\hline
ResNet101-E20 & \acronym{RM;GN}     & 2.508      & 2.827       & 0.319 &-\\
                     & \acronym{RM;RN}     & 0          & 0.424     & 0.424 &0.424\\
                     & O (1) RM;RN         & -          & -     & - &0.505\\
\hline
ResNet101-E100 & \acronym{RM;GN}     & 2.508      & 3.47       & 0.962 &-\\
                     & \acronym{RM;RN}     & 0          & 1.03     & 1.03 &1.03\\
                     & O (1) RM;RN         & -          & -     & - &1.40\\
\hline
% ResNet101-E50 & \acronym{RM;GN}     & 2.508      & 3.151       & 0.643 &-\\
%                      & \acronym{RM;RN}     & 0          & 0.610     & 0.610 &-\\
%                      & O (1) RM;RN         & -          & -     & - &0.81\\
% \hline

GPT2-E12 & \acronym{RM;GN}     & 3.78      & 3.47     & 0 &-\\
                     & \acronym{RM;RN}     & 0          & 0.30    & 0.30 &0.30\\
                     & O (1) RM;RN         & -          & -    & - &1.54\\
\hline
GPT2-E23 & \acronym{RM;GN}     & 3.78      & 3.96     & 0.18 &-\\
                     & \acronym{RM;RN}     & 0          & 1.15    & 1.15 &1.15\\
                     & O (1) RM;RN         & -          & -    & - &2.54\\
\hline
GPT2-E46 & \acronym{RM;GN}     & 3.78      & 4.07    & 0.29 &-\\
                     & \acronym{RM;RN}     & 0          & 2.37   & 2.37 &2.37\\
                     & O (1) RM;RN         & -          & -    & - &4.12\\
\hline
GPT2-E92 & \acronym{RM;GN}     & 3.78     & 5.06    & 1.28 &-\\
                     & \acronym{RM;RN}     & 0          & 3.45    & 3.45 &3.45\\
                     & O (1) RM;RN         & -          & -    & - &5.43\\
\hline
MLP Tabular-E100 & \acronym{RM;GN}     & 1.25      & 1.62     & 0.37 &-\\
                     & \acronym{RM;RN}     & 0          & 0.64       & 0.64 &0.64\\
                     & O (1) RM;RN         & -          & -       & - &0.22\\
\hline
\end{tabular}}
 \caption{\acronym in comparison to privacy auditing with O(1) training.}
\label{o1_rmrn_metrics}
\end{table}
We evaluate the effectiveness of our technique in detecting privacy leakage from ML models, by comparing \acronym with \cite{steinke2023privacy} Privacy Auditing with One (1) Training Run.  \cite{steinke2023privacy}'s auditing framework is well suited to ours in terms of comparison owed to their significant contribution of reducing the number of training runs required to audit an ML model from the order of thousands to only one. We aim to bring these re-training runs of the target model needed to conduct the audit down to zero, while also replacing the dependency of having real non-member data available to conduct the audit. Hence the O(1) privacy audit is a natural choice for comparison with our results. Given our baseline provides an adequate estimate/bound on $c-closeness$ of the synthetic non-member data to the real member data distribution, we expect the $\epsilon$ returned by \acronym while auditing the target on real member and generated non-member data to be close to O(1) auditing the target on real member and real non-member data. We also present the case where \acronym deals with real member and real non-member data. 
We conduct the O(1) privacy audit following the algorithm provided by \cite{steinke2023privacy}, with members, and non-members classified as a positive and negative guess $\{+1, -1\}$ respectively, and $0$ for abstentations. The experimental details for each data modality can be found in appendix \ref{appendix:O1_exp_details}.

As shown in table \ref{o1_rmrn_metrics}, the privacy loss values returned by \acronym and auditing with O(1) training runs are reasonably comparable: both \acronym and O(1) detect leakage of the same order of magnitude and this value increases when the value of overfitting with respect to model training epochs increases, categorizing more memorization of the respective ML model. It is interesting to note that O(1) provides a slightly higher value of $\epsilon$ as opposed to \acronym, both in the case where \acronym deals with generated non-members (GN), as well as real non-members (RN). The key difference in terms of how we measure privacy leakage is that we consider only members, i.e. we only count positives in our analysis, as opposed to members and non-members (both positive and negative guesses) in the case of O(1). As \acronym is an ML-based MIA attack that trains on both raw image data as well as loss values of target model $f$ on this data, it is expected to outperform O(1) in some cases if the signal from data combined with the target model's loss contains more information that using only the loss. We observe such a case in the tabular dataset for extreme overfitting, in the case of 100 training epochs of the MLP model on the adult dataset. 
\todo{Justify with numbers for v and r in cases O(1) outperforms and justify with accuracy (v/r) where Panoramia outperforms
\\
- - some detail on Panoramia RM;RN = perfect generator, so eps tilda=eps.}


\subsection{ Target Model Trained on Real Data and Synthetic Data as Canaries}

\begin{table}
  \centering
  \resizebox{0.5\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Target model} & \textbf{Audit} & $\mathbf{c_{lb}}$ & $\mathbf{\varepsilon + c_{lb}}$ & $\mathbf{{\varepsilon}}$ \\
\hline
ResNet101-E20     
                     & \acronym{RMGM;RNGN} & 0          & -   & 0.731 \\
                     & O (1) RMGM;RNGN    & -          & -     & 0.817 \\
\hline
ResNet101-E100     
                     & \acronym{RMGM;RNGN} & 0          & -   & 1.57 \\
                     & O (1) RMGM;RNGN    & -          & -     & 1.92 \\
\hline
GPT-2 E12     
                     & \acronym{RMGM;RNGN} & 0          & 0.32  & 0.32 \\
                     & O (1) RMGM;RNGN    & -          & -     & 1.23\\
\hline
GPT-2 E23     
                     & \acronym{RMGM;RNGN} & 0          & 1.17  & 1.17 \\
                     & O (1) RMGM;RNGN    & -          & -     & 2.07\\
\hline
GPT-2 E46     
                     & \acronym{RMGM;RNGN} & 0          & 2.27  & 2.27 \\
                     & O (1) RMGM;RNGN    & -          & -     & 3.27\\
\hline
GPT-2 E92     
                     & \acronym{RMGM;RNGN} & 0          & 3.01   & 3.01 \\
                     & O (1) RMGM;RNGN    & -          & -     & 4.78\\
\hline



MLP Tabular-E100     
                     & \acronym{RMGM;RNGN} & 0          & -   & 0.49 \\
                     & O (1) RMGM;RNGN    & -          & -     & 0.37 \\
\hline
\end{tabular}}
\caption{\acronym in comparison to privacy auditing with O(1) training when auditing target model with synthetic canaries added to the training dataset.} 
% \ali{Why is O(1) in $\mathbf{\tilde{\varepsilon}}$ column?} \mishaal{i fixed it, thanks!}
\end{table}

We also evaluate the performance of \acronym on a target model where we add synthetic "canaries" into the member dataset of the ML model's original train set. With this we aim to assess how \acronym performs in comparison to O(1), when we have the case of a "perfect" generator, in that members and non-members both are from the same distribution, i.e. they can be from both the synthetic data or real data, hence baseline returns $c=0$. 
We observe that the privacy loss values returned by both auditing frameworks increase; this is expected as detecting canaries, is relatively easier in comparison to real data of the same distribution. 

- exp details: model, data split for RM; GN; test accuracy, test set, params, etc.
- note the effect of adding canaries has on the audit of the target model

==> src/baseline_eval.tex <==
\section{Baseline Classifier Strength Evaluation}
The basis of our audit directly depends on how well our baseline classifier distinguishes between real member data samples and synthetic non-member data samples generated by our generative model. To certify the strength of the baseline classifier, we train the baseline's helper model $\helper$ on various datasets
\ali{Here, it should be more clear that what are these various datasets. Also, it should be more clear that only for the sake of this comparison, we keep some real samples as non-member, not anywhere else in the experiments.}
and report the $c_{lb}$ for each case. The results in table \ref{table:baseline_eval} show the comparison of baseline helper trained on real data of the same distribution as the respective target ML model, generated data produced by our generative models in each respective data modality setting, as well as a mix of half and half of real and generated data to train the helper model.
In addition, we also experiment with different helper model architectures. The baseline with the highest $c_{lb}$ is chosen for each data modality setting.
\ali{We need a conclusion or takeaway sentence here to conclude that a helper trained with synthetic data is sufficient, no need for real non-members.}
This value works two-fold \ali{What's the second point?}: it allows us to get a tight worst-case lower bound \ali{Isn't it a strong claim to say it's tight?} on how close the generated non-member data is to the real member data distribution.
We also choose the setting that returns the highest $c_{lb}$ and train that baseline on an increasing dataset size of member and synthetic non-member data to gauge the trend of the baseline performance as the training dataset size increases. The experiments are repeated ten times to account for randomness during training (e.g. initialization, sampling in batches) and report the results over a $95\%$ confidence interval. We choose the train dataset size for our MIA and baseline where the performance of the baseline plateaus or stabilizes.  \ali{we should be more clear on the connection of this to the table 3 $\clb$, and also expalin if we change the experiment setup for this result}
\begin{figure*}[bp]
  \centering
  
  \subfigure[$c_{lb}$ as training data increases for baseline trained to distinguish real and synthetic CIFAR10 image data points.]{\includegraphics[width=0.33\linewidth]{ICML24/images/baseline_cifar10_clb.pdf}\label{subfig:image1}}
  \hfill
  \subfigure[$c_{lb}$ as the size of the training set increases for baseline, trained to distinguish real (WikiText-2) and synthetic data points.]
     {\includegraphics[width=0.33\linewidth]{ICML24/images/nlp_baseline_plateau.pdf}}
  \hfill
  \subfigure[$c_{lb}$ as training data increases for baseline trained to distinguish real and synthetic Adult tabular  data points.]{\includegraphics[width=0.33\linewidth]{ICML24/images/tab_c_lb_trainingsize_full.pdf}}
  
  \caption{Baseline strength evaluation as the training dataset size of the baseline classification model increases. } 
  
  \label{fig:three_images}
\end{figure*}

\begin{table} [h]
\centering
 \resizebox{0.30\textwidth}{!}{
\begin{tabular}{|l|l|}
\hline
Baseline model                               & \(c_{lb}\) \\
\hline
CIFAR-10 Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{real, resnet101}\)} & 2.16 \\
CIFAR-10 Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{imgnet}\)}          & 1.10 \\
CIFAR-10 Baseline\textsubscript{no helper}                                    & 1.15 \\
CIFAR-10 Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{real, WRN}\)}      & 2.37 \\
CIFAR-10 Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{gen, WRN}\)}       & \textbf{2.508} \\
\hline
WikiText-2 Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{gen}\)}      & \textbf{2.61} \\
WikiText-2 Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{real}\)}      & 2.59 \\
WikiText-2 Baseline\textsubscript{no helper}                                    & 2.34 \\
\hline
Adult Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{gen}\)}      & \textbf{2.34} \\
Adult Baseline\textsubscript{\(D_{h}^{\text{tr}}=\text{real}\)}      & 2.18 \\
Adult Baseline\textsubscript{no helper}                                    & 2.01 \\
\hline
\end{tabular}}

\caption{Baseline evaluation with different helper model scenarios 
}
\vspace{-10pt}
\label{table:baseline_eval}
\end{table}


==> src/conclusion.tex <==
With \acronym, our work introduces a brand new capability in the ML auditing toolbox: the ability to audit trained ML models (not only training algorithms) for privacy leakage of samples from a specific data distribution for a subset of the training set (\emph{e.g.}, the data distribution of one participant in a FL model; or of a sub-population of interest), with access to only the trained model to audit, and a dataset of members of the training set from the distribution of interest.
\acronym does not require access to the training procedure, the full training set, or non-member data from the same distribution. 
It does not assume control of the training procedure (\emph{e.g.}, to add canaries), neither does it require changing the final model or retraining new (shadow) models.
\acronym is thus a practical approach to quantifying privacy leakage, in settings previously not amenable to privacy audits.
We also believe that this new capacity can enable applications outside of direct ML privacy audits, such as the passive detection of unintended data uses, as in \cite{lecuyer2014xray, lecuyer2015sunlight}. %\ml{kind of citing my own work, we can remove if better, but I that'd be a very cool thing to do!} \ml{other ideas?}

As a first proposal for privacy audits without retraining, \acronym leaves several technical questions open, that would benefit from further work and expand the capability of no retraining privacy audits.
The main limitation of our approach is that the privacy loss we measure is not a proper lower-bound (see \S\ref{subsec:dp-measurement}). 
Ideally, the hypothesis test would provide an upper-bound on $c$, potentially with a failure probability akin to DP's $\delta$. 
This seems challenging in the general case of a distribution: could we refine \acronym's analysis to only focus on the audited sample, and provide an upper-bound for $c$ in this context? This would have the added benefit of auditing privacy loss for a specific data subset, and not a distribution of a subset. It would also become meaningful to audit $(\epsilon, \delta)$-DP.
Another promising direction is to develop better generators for $c$-closeness, that also favor membership inference to strengthen the privacy audit, as well as better statistical tests.
Overall, we believe that \acronym introduces an important new capability for practical privacy audits, with several open directions to expand this capability.

%With our work, we propose a new auditing mechanism, \acronym, that offers practicality to industry and high-stake domains in terms of adoption and deployment by removing the need for resampling and retraining ML models in the process. Our results with high confidence, show that the MIA via non-member synthetic data can provide an avenue to do so. Following previous literature, we show that our privacy auditing mechanism catches the nature of complex models with more parameters in that they memorize more data and have more information on the training data points as compared to simple deep nets. Having information on the ML model gives an advantage to the attacker. 

%We believe that our approach, when improved upon with future work discussed above, can be used to lower-bound the privacy loss incurred by training an ML model (through an empirical counter-example), which could complement an upper-bound given by DP theory as well as provide a practical auditing scheme in large-scale federated learning systems without the need to retrain large ML global model pipeline from scratch.

==> src/empirical.tex <==



We instantiate \acronym on target models for four tasks from three data modalities: two image classification tasks, one language modeling task with a large language model (LLM) target, and a classification task on tabular data. 
Table \ref{table_metrics} summarizes the task, datasets, and target model architectures audited for each modality. 

\subsubsection{Generator.} 
We generate synthetic data that serves as non-members for our attack using the StyleGAN2~\cite{karras2020training} to train the generative model $\gG$ for the image datasets, the  MST algorithm \cite{mckenna2021winning} for the tabular dataset. In the text data setting, the generative model $\gG$ is based on a small GPT-2, fine-tuned using a CLM task on dataset $\DG$.  In each case, generative model $\gG$ is trained on one-third of the dataset used to train the audited model $ \DG \subseteq D_f $. 
Figure~\ref{datasets} shows member and non-member images used in our experiments for the image classification task.

\subsubsection{Baseline \& MIA.}
For the MIA we follow a loss-based attack approach, in that \acronym takes as input raw member and non-member data points for training along with the loss values the target model $f$ attributes to these data points.
More precisely, the training set of \acronym is:
\[(D^{tr}_{in}, f(D^{tr}_{in}) \cup  (D^{tr}_{out}, f(D^{tr}_{out})\]
In \S\ref{subsec:dp-measurement}, we discussed the importance of having a tight $\clb$ so that our measure, $\tilde\epsilon$, becomes close to a lower-bound on $\epsilon$-DP. This requires a strong baseline. 
To strengthen our baseline, we introduce the helper model $\helper$, which helps the baseline model $b$ by supplying additional features (\emph{i.e.}, embeddings) that can be viewed as side information about the data distribution.
The motivation is that \helper's feature might differ between samples from $\gD$ and $\gD'$, enhancing the performance of the baseline classifier.

For each modality, we  describe the task, datasets, and target model architectures audited (summarized in Table \ref{table_metrics}), the generators used, and the architecture and settings for the baseline model and \acronym's MIA models in more detail in appendix \ref{exp_details}.

\subsection{Privacy Auditing using \acronym}

\textbf{Interpretation of the Baseline $\mathbf{c_{lb}}$}: 
Recall that \acronym relies on the quality of synthetic data to measure privacy loss. This quality is assessed by the baseline, from which we can compute $\clb$, a lower bound on $c$-closeness for $\gG$.
%
Focusing on the blue line for the baseline, Figure~\ref{fig:comparison_precision} shows the precision-recall curve for the task of membership inference (looking only at raw data and helper model's embedding for the baseline).
For each value of recall on the x-axis, the precision achieved by the baseline coupled with Proposition \ref{prop:gen-test} and Corollary \ref{result:confidence-interval} gives a lower bound for $c$, shown in Figure~\ref{fig:comparison}.
Figure \ref{fig:elb_comparison} decomposes the precision in numbers of true positives and the number of predictions for a direct mapping to the propositions. Following lines \ref{algo:max-t-start}-\ref{algo:max-t-end} in the last section of Algorithm \ref{algo:panoramia} and the associated discussion in \S\ref{sec:theory}, we pick the largest lower-bound implied at any recall, $\clb$, shown as the dashed blue line on Figure~\ref{fig:comparison}. The associated upper bound on precision at a recall is shown with a dashed line in Figure~\ref{fig:comparison_precision}.

\textbf{Interpretation of the MIA Results}
Having established the value of $\clb$, we proceed to the second part of the hypothesis testing, using Proposition \ref{prop:dp-test} and Corollary \ref{result:confidence-interval} to measure $\{c+\epsilon\}_\textrm{lb}$.
Figure~\ref{fig:comparison_precision} presents the precision-recall curve of $\acronym$'s MIA for different target models from Table \ref{table_metrics}. 
For both image datasets, we can see that the precision-recall curves obtained by the MIA are above the one from the baseline. In other words, the addition of information from the audited model $f$ leads to better performance when distinguishing between real and synthetic images.
We observe similar behavior on the tabular dataset and WikiText-2 data. 

Similar to $c$-closeness, we leverage the obtained precision for a given number of guesses to compute the maximum value of $\cpepslb$, presented in figure \ref{fig:comparison}.
For all datasets, we obtain maximum values of $\cpepslb$ greater than $\clb$. 
%except GPT-2\_E12, 
% Ali: the above line is not relevant anymore.

The value of $\tilde\epsilon$ for each target model is the gap between its corresponding dashed line and the baseline dashed line. 
This allows us to compute values of $\tilde\epsilon$ reported in Table \ref{table:audit_values}.

%\hadrien{add a few sentences to describe this table when finished}
%For all experiments, we notice that more training epochs on the audited model lead to greater values of $\{c+\epsilon\}_\textrm{lb}$ Our experiment is coherent with the intuition that more training epochs lead to more over-fitting which in turn leads to more privacy leakage. 
It is also interesting to note that the maximum value of $\cpepslb$ typically occurs at low recall. 
Even if we do not use the same metric (precision-recall as opposed to TPR at low FPR) this is coherent with the findings from \citet{carlini2022membership}. We can detect more privacy leakage (higher $\cpepslb$ which leads to higher $\tilde\epsilon$) when making a few very confident guesses about membership rather than trying to maximize the number of members found (recall). Table \ref{table:audit_values} collects the value of $\cpepslb$, as well as $\tilde\epsilon = \cpepslb - \clb$ measured by \acronym. We can see that $\tilde\epsilon$ reaches up to $0.962$ on Cifar-10 (ResNet101\_E100), $1.02$ on CelebA (Multi-Label CNN-E100), $1.28$ on WikiText-2 (GPT-2\_E96), and $1.34$ on Adult (MLP\_E100). 

These are non-negligible values of privacy leakage, even though the true value is likely much higher.

We also report in table \ref{table:audit_values}, the values returned by auditing the target model using \cite{steinke2023privacy}'s framework for Privacy Auditing with One (1) Training Run. We discuss these numbers in detail in section...., for now, we observe that the privacy loss values obtained by both frameworks are comparable and close to one another making \acronym a strong tool in the privacy auditing domain without requiring the need for retraining the ML model. 

\subsubsection{\acronym and Auditing Models of Varying Overfitting}
In Figure \ref{fig:comparison_precision}, we observe that more training epochs (more overfitting) lead to better precision-recall trade-offs and higher maximum precision values. Our results are further confirmed by figure \ref{fig:elb_comparison} with \acronym being able to capture the number of member data points better than the baseline $b$.
We report the train and validation loss as a measure of overfitting in figure \ref{fig:gpt-2-target-overtraining-loss}.
Figure~\ref{fig:gpt_losses} shows how the gap between member data points (\emph{i.e.}, data used to train the target models) and non-member data points (both real as well as generated non-members) increases as the degree of overfitting increases, in terms of loss distributions.
In table \ref{table:audit_values}, we further demonstrate that our audit output $\tilde\epsilon$ orders the target models in terms of privacy leakage: higher the degree of overfitting, more memorization and hence a higher $\tilde\epsilon$ returned by \acronym. 
From our experiments, we consistently found that as the number of epochs increased, the value of $\tilde\epsilon$ also increased. 
Our experiments are therefore coherent with previous literature that increasing the number of training epochs for the target model to induce overfitting is known to be a factor in privacy loss \cite{yeom2018privacy, LIRA}. \\

\textbf{Investigating cases where \acronym may return no privacy leakage} \\
% There are also cases in which \acronym is not able to meaningfully measure privacy loss.
% For instance, the precision-recall curves of both the baseline (blue) and \acronym's MIA for GPT-2\_E23 have similar maximum precision values. As a result,  the maximum value for $\cpepslb$ is close to $\clb$ (figure \ref{fig:gpt2_privacy_recall} ) leading to a small $\tilde \epsilon$ value even if the MIA outperforms the baseline. This is due to our independent selection of recall thresholds, which leads to similar maximum values of $\clb$ and $\cpepslb$.
% Ali: the above is not super relevant anymore, at least not with the new GPT-2 results
As illustrated in Figure \ref{fig:gpt2_privacy_recall}, there exist instances where the $\clb$ is as large or even larger than $\cpepslb$ (such as in GPT-2\_E12). This implies that, under certain conditions, the baseline could outperform the membership inference attack in \acronym. We can see three primary reasons for this behavior:  (1) The synthetic data might not be of high enough quality. If there is an evident distinction between real and synthetic samples, the baseline cannot be fooled reducing the power of our audit. (2) The MIA in \acronym is not powerful enough. (3) The target model's privacy leakage is indeed low \ali{mention that this target model indeed has the lowest validation loss} \ali{Also, we should discuss the difference to O(1), and argue that O(1) rely on negative predictions}. For GPT-2\_E92, GPT-2\_E46, and GPT-2\_E23 \ali{GPT-2\_E23 is kinda low-ish, so not sure if it fits in this argument} in Figure \ref{fig:gpt2_privacy_recall}, we can claim that given the target model's leakage level, the synthetic data and the MIA can perform the audit to a non-negligible power. For GPT-2\_12, we need to examine the possible reasons more closely.
We discuss this case and the reasoning in more detail in appendix  \ref{subsec:no-priv-leak}. 


\subsubsection{\acronym and Privacy Auditing of Differentially Private Models}

% {\bf Methodology.} 
We evaluate the performance of \acronym on differentially private (DP) ResNet-18 models on the CIFAR10 dataset under different target privacy budgets ($\epsilon$) and the non-private ($\epsilon=\infty$) cases. The models are trained using the DP-SGD algorithm \citep{abadi2016deep} which we tune each one independently for the highest train accuracy. We include more results and discussions in Appendix \ref{appendix:dp_sup_results}.

% {\bf Results.} 




Table \ref{tab:dpResNet18-table}, and the accompanying $\{c+\epsilon\}$ vs recall plot, figure \ref{subfig:resnet18-dp-fig} shows that at $\epsilon=2$ (a more private model) \acronym suggests no privacy leakage is detected, whereas at higher values of $\epsilon=10,15$ (less private models) and $\epsilon=\infty$ (a non-private model) \acronym detects an increasing level of privacy leakage with $\tilde{\epsilon}_{\epsilon=10} < \tilde{\epsilon}_{\epsilon=15} < \tilde{\epsilon}_{\epsilon=\infty}$, suggesting a higher value of $\epsilon$ correspond to higher $\tilde \epsilon$. We compare the performance of \acronym with that of privacy auditing with O(1) training runs \citep{steinke2023privacy}. The conclusion between the two methods is comparable, in which no privacy leakage is detected at $\epsilon=2$ and higher privacy leakage is detected at $\epsilon=10,15,\infty$.


\mishaal{varying complexities + dp plot in double 1 column added in figure 2 above}

\subsubsection{\acronym and Privacy Auditing of Models with Varying Complexity}
 We also consider the behavior of our privacy auditing mechanism in the case of models with varying complexities for image classification models. 
 We categorize the complexity of these models in terms of the number of parameters with the Wide ResNet-28-2 having approximately 35,616 parameters (least complex), followed by the ResNet-50 with approximately 3,123,360 parameters, \mishaal{fix this} and then the ResNet-101 being relatively most complex with approximately 3,123,360 parameters.

 We Achieve perfect ordering in terms of model complexity: a more complex model memorizes and therefore leaks more data than a less complex one. As shown in Figure \ref{subfig:var_complexities}, ResNet101 being the most complex model leaks the most information as opposed to the relatively least complex Wide-ResNet-28-2.  This trend is consistent in terms of $\Tilde{\epsilon}_{wide-resnet} \leq \Tilde{\epsilon}_{resnet50}\leq \Tilde{\epsilon}_{resnet101}$. Therefore, with \acronym we capture the degree of model complexity in relation to an ordering in terms of privacy leakage attributed to that model, confirming claims of previous research. \mishaal{reference}
 


\section{Experimental Setting (Actual)}

\mishaal{actual section 6 (untouched)}

We instantiate \acronym on target models for four tasks from three data modalities: two image classification tasks, one language modeling task with a large language model (LLM) target, and a classification task on tabular data. 
For each modality, we next describe the task, datasets, and target model architectures audited (summarized in Table \ref{table_metrics}), the generators used, and the architecture and settings for the baseline model and \acronym's MIA models.

% In this section, we demonstrate the effectiveness of \acronym~on ML models handling three types of data modalities, namely image classification models, LLMs as well as classification models on tabular data.
% %Seb: we need to be sure the acronym LLM has been defined previously

\subsection{Image Classification}

{\bf Target models.} We audit target models with three architectures: a Multi-Label Convolutional Neural Network (CNN) with four layers \cite{oshea2015introduction}, and the ResNet101 \cite{he2015deep}. We also include in our analysis, differentially private models for ResNet18 \cite{he2015deep} and WideResNet-16-4\cite{zagoruyko2017wide} models as targets, with $\epsilon = 1, 2, 4, 6, 10, 15$ and $\epsilon =20$. 
The ResNet-based models are trained on Cifar10 using $50k$ images \cite{Krizhevsky2009LearningML} of $32$x$32$ resolution. The Multi-Label CNN is trained on $200k$ images of CelebA \cite{liu2015faceattributes} of $128$x$128$ resolution to predict $40$ attributes associated with each image.

{\bf Generator.} For both image datasets, we use StyleGAN2~\cite{karras2020training} to train the generative model $\gG$ from scratch on $\DG$, and produce non-member images. 
Generated images will in turn serve as non-members for performing the MIAs. 
Figure~\ref{datasets} shows member and non-member images used in our experiments.

\textbf{Baseline \& MIA.}
For the MIA we follow a loss-based attack approach, in that \acronym takes as input raw member and non-member data points for training along with the loss values the target model $f$ attributes to these data points.
More precisely, the training set of \acronym is:
\[(D^{tr}_{in}, f(D^{tr}_{in}) \cup  (D^{tr}_{out}, f(D^{tr}_{out})\]
In \S\ref{subsec:dp-measurement}, we discussed the importance of having a tight $\clb$ so that our measure, $\tilde\epsilon$, becomes close to a lower-bound on $\epsilon$-DP. This requires a strong baseline. 
To strengthen our baseline, we introduce the helper model $\helper$, which helps the baseline model $b$ by supplying additional features (\emph{i.e.}, embeddings) that can be viewed as side information about the data distribution.
The motivation is that \helper's feature might differ between samples from $\gD$ and $\gD'$, enhancing the performance of the baseline classifier.
%
This embedding model $\helper$ is similar in design to $f$ (same task and architecture) but is trained on a different dataset from the same distribution $\gD$.
%More precisely, $e$ is trained to generalize well, making $e$ generate consistent embeddings across its training dataset and $\DT$. 
%Essentially, $e$ should produce similar features throughout the $\gD$ distribution.
%However, when considering the synthetic data from $\gG$, $e$'s embeddings might differ. 
%We leverage this discrepancy to
Whether for the baseline or MIA, we use side information models ($\helper$ and $f$, respectively) by concatenating the loss of $\helper(x)$ and $f(x)$ to the final representation, before a last layer makes the membership the prediction. %(see Appendix \ref{app}
Since we need labels to compute the loss, we label synthetic images with a basic classifier (a vanilla CNN) trained on a subset of the data. % separate from the member data of $f$, to get the losses of $f$ for the synthetic data.

In all other aspects, the MIA and baseline $b$ have the same ResNet101 architecture. More details can be found on training MIA and baseline in appendix section \ref{subsec:imgexpdetails}.

%Seb: I put this in comments as it was incomplete
%Based on these, \acronym gives us precision and recall values that we use to 
% \subsubsection{Image classification models.}
% \acronym~is evaluated on ResNet50, ResNet101, and Wide ResNet-28-2 models trained on 30,000 images of the CIFAR10 dataset (32x32 resolution).
% Our privacy auditing framework is also assessed on a Multi-Label CNN, with 4 convolutional layers and 3 fully connected layers trained on 25,000 images of the CelebA dataset (128x128 resolution). 
% Each image in the CelebA dataset has 40 attributes (\emph{i.e.}, labels) associated with it. 
% StyleGAN2~\cite{karras2020training} is used as the generative model to produce non-member images for both these image datasets, which in turn will serve as non-member or out data points for performing the MIAs. 
% Figure~\ref{datasets} displays a comparison of member and non-member images used in our experiments.

\begin{figure}[htbp]
  \centering
  \subfigure[Real]{\includegraphics[width=0.11\textwidth,height=0.6604in]{ICML24/images/celebAreal_2.png}
  \label{subfig:celebAreal}}
  \hfill
  \subfigure[Synthetic]{\includegraphics[width=0.11\textwidth,height=0.6604in]{images/celebFake_2.png}
  \label{subfig:celebFake}}
  \hfill
  \subfigure[Real]{\includegraphics[width=0.1\textwidth]{ICML24/images/cifarReal_2.png}
  \label{subfig:cifarReal}}
  \hfill
  \subfigure[Synthetic]{\includegraphics[width=0.1\textwidth]{images/cifarFake_2.png}
  \label{subfig:cifarFake}}
  \caption{Member and Non-Member datasets used in our experiments for CelebA (\ref{subfig:celebAreal}, \ref{subfig:celebFake}) and CIFAR10 (\ref{subfig:cifarReal}, \ref{subfig:cifarFake}) image data. } 
  \label{datasets}
\end{figure}





\subsection{Language Modeling}
\label{subsec:llmexpsetting}
{\bf Target model.} The target model is a model fine-tuned for the causal language modeling (CLM) task.
We start from a pre-trained small GPT-2~\cite{radford2019language} language model, and fine-tune it on WikiText-2 train dataset \cite{merity2016pointer}, a collection of Wikipedia articles. 
While the GPT-2 training dataset is undisclosed, \cite{radford2019language} do state that they don't include any Wikipedia document. 
We also incorporate a few additional documents from WikiText-103 (the larger version of the WikiText dataset) into $\DT$ to augment $\Dinte$, enabling us to estimate bigger values for $\clb$ and $\{c+\epsilon\}_\textrm{lb}$.
Moreover, for comparing \acronym to O(1) auditing method (discussed in section \ref{sec:O(1)}), we need to keep a subset of the available WikiText samples as non-members, leading to the target model not being trained on the entire real dataset that we have. Additionally, O(1) method necessitates random inclusion/exclusion of samples into the target model train set \cite{steinke2023privacy}. Consequently, the samples within $\DT$ may be from either WikiText-2 or WikiText-103. Although \acronym requires no adjustments to the pipeline, we modify the training pipeline solely for the purpose of comparing it to the O(1) method. 

% it is presumed to be substantial, potentially containing the entirety of the WikiText-2 dataset. 
% Hence, by fine-tuning GPT-2 on this dataset (\emph{i.e.}, not training from scratch), we might not have access to any real non-member sample. 
% However, this is not an issue in \acronym since the non-member data is created synthetically. 


{\bf Generator.}
Our generative model $\gG$ is again based on small GPT-2, fine-tuned using a CLM task on dataset $\DG$. 
To create synthetic samples with $\gG$, we use top-$p$ sampling~\cite{holtzman2019curious}.
%Seb: eventually, we might provide more details about how top-p sampling works
To generate better samples, we split the $\DG$ dataset into two parts: $\DG^{train}$ and $\DG^{prompt}$.
$\gG$ is fine-tuned on $\DG^{train}$, while $\DG^{prompt}$ is used for generating prompts.
During generation, we take a sample from $\DG^{prompt}$, 
%grab the first $k$ tokens, 
and request the generator to independently produce multiple sequences, each of which is of equal length to the input prompt. In experiments, 
% we use $k=32$, and 
each generated sample is of the length of $64$ tokens, and we generate 5 synthetic samples per one prompt.
Note that this generation approach does not inherently favor our audit scheme, and shows how \acronym can leverage existing, public generative models with fine tuning to access high-quality generators at reasonable training cost.
%SebL ideally, we should have some arguments to motivate why 32 is a good number
%Ali: I have some figures regarding that. I would include it in the appendix, if I got time. 
%Ali: The generation process in which I take only the first k tokens of a prompt got changed. Now I give the whole prompt.

\textbf{Baseline \& MIA.}
For both the baseline and \acronym~classifiers, we use a GPT-2 based sequence classification model. 
In this setup, GPT-2 extracts a feature representation (\emph{i.e.}, hidden vector) directly from the sample's text.
To this representation, we concatenate a vector of features extracted using the helper embedding $\helper$ (for the baseline) or target model $f$ (for the MIA). This vector of features is the loss sequence produced in a CLM task for the respective model.
The final concatenated representation goes through one layer for the final prediction.
For both the baseline and \acronym~classifiers,
the training and validation sets consist of 12000 and 2000 samples, respectively, with equal member non-member distribution. The test set consists of 10000 samples, where the actual number of members and non-members that ended up in the test set depends on the Bernoulli samples in the auditing game.
% the training and validation sets each comprise 1000 samples (500 samples per member/non-member class) while the test set consists of 2000 samples. 
Full details are given in Appendix~\ref{subsec:llmfullexpdetails}


\subsection{Tabular Data Classification.}
{\bf Target model.}
For tabular data, we evaluate our attack on a Multi-Layer Perceptron (MLP) with 4 hidden layers trained on the Adult dataset. We perform a binary classification task, predicting whether an individual earns more than \$50k annually. 
$\DT$ is one-half of the Adult Dataset.

{\bf Generator.} 
We generate synthetic tabular data using the MST algorithm \cite{mckenna2021winning} trained on the same dataset used to train the audited model %$ \DG \subseteq D_f $.
%The original dataset is divided into two halves, with the first half being used to train the audited model $f$, while the second one is used to train a classifier.

\textbf{Baseline \& MIA.}
To distinguish between real and synthetic data, we use a gradient boosting model for both baseline and MIA. 
%
Similarly to the image and text modalities, we provide additional information to the baseline for the tabular case using an helper model $\helper$ trained on synthetic data.
%And in the case of MIA, we provide the embedding from the target model $f$.
In the case of tabular data, the embedding simply consists of the loss from either $\helper$ or $f$, where $\helper$ has the same architecture as $f$.% but is trained on a different dataset $D_h \nsubseteq D_f$ from $\mathcal{D}$. This embedding is added to the raw data as a new feature.
\mishaal{Hadrien can u please re-word the above for more clarity}
%The baseline model takes as input raw data and embedding $e$ while the MIA uses raw data and the loss from the target model $f$.




\begin{table*} [t]
    \centering
     \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        ML Model & Dataset & Training Epoch  & Test Accuracy &  Model Variants Names* \\
        \hline
        ResNet101 &CIFAR10 & 20, 50, 100  & 91.61\%, 90.18\%, 87.93\%& ResNet101-E20, ResNet101-E50, ResNet101-E100,\\
        % Wide ResNet-16-4 & CIFAR10 & 20, 50, 70  & \%, \%, \% & W-RN\_E20, W-RN\_E70, W-RN\_E100 \\
        Multi-Label CNN & CelebA & 50, 100  & 81.77\%, 78.12\% & CNN\_E50, CNN\_E100 \\
        GPT-2 & WikiText-2 & 12, 23, 46, 92 & Refer to Figure \ref{fig:gpt-2-target-overtraining-loss} & GPT-2\_E12, GPT-2\_E23, GPT-2\_E46, GPT-2\_E92 \\
        MLP Tabular Classification  & Adult & 10, 100 & 86\%, 82\%  & MLP\_E10, MLP\_E100\\
        \hline
    \end{tabular}}
    \caption{Train and Test Metrics for ML Models Audited. *"Model Variants" refers to the models audited at varying numbers of training epochs $E$, with the respective names used in plots.}
    \label{table_metrics}
    %\mishaal{update table wrt new numbers}\ml{the table is too wide, we can't have that in the paper it won't pass the format check} \mishaal{is it okay now?} \ml{yes}
\end{table*}

==> src/results.tex <==
% \section{Results} 


%\ml{The goal of this section is to demonstrate when \acronym works, and show/discuss when it doesn't as well. We have two main subsections, and each can have a small {\bf Methodology:} and a few paragraph on that (keep it short if possible), and then {\bf Results:} and you do the results paragraphs. Keep it symmetric so it's not too confusing!}

We use our instantiating of \acronym from \S\ref{sect_exp} to evaluate the quality of \acronym's privacy leakage assessments. We first show precision-recall plots for the baseline and MIA on several target models, and explain how to interpret them in the context of \acronym's hypotheses tests to measure privacy leakage (\S\ref{subsec:general-results}). We then focus on three dimensions known to influence privacy leakage: overfitting (\S\ref{sect_results_overfitting}), model size (\S\ref{sect_results_overfitting}), and DP training (\S\ref{subsec:eval:dp-target}). In each case, we verify that \acronym can properly detect and order variations in the privacy loss.

%\ml{I think this subsection should move to the next section and be merged with the methodology for the first results subsection where Hadrien suggested it. This section is for the audits we did, this part is more related to the evaluation methodology (we want different levels of privacy leakage to assess how well \acronym works)}

% \begin{figure*}
%   \centering
%   \subfigure[CelebA Multi-Label CNN\_E30.]{\includegraphics[width=0.48\linewidth]{images/celebs_losses_overfit_30_True.pdf}}
%   \hfill
%   \subfigure[CelebA Multi-Label CNN\_E100; an overfit model.]{\includegraphics[width=0.48\linewidth]{images/celebs_losses_overfit_100_True.pdf}}
%   \subfigure[GPT-2\_E12]{\includegraphics[width=0.48\linewidth]{images/nlp_loss_separability_target_E12_wt2_gen_config6.pdf}
%   \label{subfig:lossdist-gpt-2E12}
%   }
%   \hfill
%   \subfigure[GPT-2\_E25]{\includegraphics[width=0.48\linewidth]{images/nlp_loss_separability_target_E25_wt2_gen_config6.pdf}
%   \label{subfig:lossdist-gpt-2E25}
%   }
%   \hfill
%   \subfigure[GPT-2\_E50]{\includegraphics[width=0.48\linewidth]{images/nlp_loss_separability_target_E50_wt2_gen_config6.pdf}
%   \label{subfig:lossdist-gpt-2E50}
%   }
%   \hfill
%     \subfigure[Embedding model $e$ ]{\includegraphics[width=0.48\linewidth]{images/nlp_loss_separability_g_wt2_gen_config6.pdf}
%     \label{subfig:lossdist-e}
%     }
%   \caption{CelebA and WikiText-2 loss comparisons for member and non-member (real and synthetic) data.}
%   \label{fig:losses}
% \end{figure*}

\begin{figure}
\vspace{-10}
  \centering
  \subfigure[CelebA Multi-Label CNN\_E30.]{\includegraphics[width=0.48\linewidth]{images/celebs_losses_overfit_30_True.pdf}}
  \hfill
  \subfigure[CelebA Multi-Label CNN\_E100; an overfit model.]{\includegraphics[width=0.48\linewidth]{images/celebs_losses_overfit_100_True.pdf}}
  \caption{CelebA Multi-Label CNN Loss Comparisons}
  \mishaal{suggestion to move this to appendix}
  \label{fig:celeb_losses}
\end{figure}

\begin{figure}
\vspace{-19}
  \centering
    \subfigure[GPT-2\_E12]{\includegraphics[width=0.45\linewidth]{images/nlp_loss_separability_target_E12_wt2_paper.pdf}
  \label{subfig:lossdist-gpt-2E12}
  }
  \hfill
  \subfigure[GPT-2\_E23]{\includegraphics[width=0.45\linewidth]{images/nlp_loss_separability_target_E23_wt2_paper.pdf}
  \label{subfig:lossdist-gpt-2E23}
  }
  \hfill
  \subfigure[GPT-2\_E46]{\includegraphics[width=0.45\linewidth]{images/nlp_loss_separability_target_E46_wt2_paper.pdf}
  \label{subfig:lossdist-gpt-2E46}
  }
  \subfigure[GPT-2\_E92]{\includegraphics[width=0.45\linewidth]{images/nlp_loss_separability_target_E92_wt2_paper.pdf}
  \label{subfig:lossdist-gpt-2E92}
  }
  \hfill
  \subfigure[Helper model $\helper$]{\includegraphics[width=0.45\linewidth]{ICML24/images/nlp_loss_separability_h_wt2_paper.pdf}
  \label{subfig:lossdist-h}
  }
  \caption{WikiText loss distributions comparison on different target models, and the helper model. \ali{Improve the caption. Explain a bit about real non-members}}
  %\caption{Loss Value Comparisons for helper model in the case of GPT-2} 
  \mishaal{suggestion to only keep generalized model and most overfit model figs here and move the rest to appendix}
  \label{fig:gpt_losses}
\end{figure}


\begin{figure}[!ht]
  \centering  
\includegraphics[width=\columnwidth]{images/nlp-GPT-2-target-overtraining.pdf}
  \caption{Target model (GPT-2) loss during overtraining on WikiText-2 dataset. We pick GPT-2\_E12, GPT-2\_E23, GPT-2\_E46, GPT-2\_E92 as target models to audit corresponding to the gray dashed lines.}
  \label{fig:gpt-2-target-overtraining-loss}
\end{figure}
\vspace{-0.07\baselineskip}


%We exploit this gap as one of the key leaking factors from our target model to detect a privacy breach in our black-box setting.
%More precisely, we rely on the fact that an ML model $f$ attributes more confident scores to data points it has encountered in its training set (lower loss) as opposed to non-member data points. 
%This offers a confident assessment that examples with high loss are non-members.  
%Figure~\ref{fig:losses} shows the fake non-members (orange) as well as real non-members (green) having a sufficient overlap in distribution to show they are interpreted by $f$ to be close in data distribution, hence leading to high-quality synthetic non-member data.



\begin{figure*}[]
    \centering
    \subfigure[Privacy Audit of ResNet-101 on CIFAR10.]{
    \includegraphics[width=0.24\textwidth]{ICML24/images/prec-recall-res101-3.png}
    \label{fig:image2}
    }
    \subfigure[Privacy Audit of a Multi-Label CNN on the CelebA dataset.]{\includegraphics[width=0.23\textwidth]{ICML24/images/celebA-prec-recall-icml.png}
    \label{fig:image3}
    }
    \subfigure[Privacy Audit of the GPT-2 on WikiText-2]{\includegraphics[width=0.23\textwidth]{images/nlp_RMFN_precision_recall.pdf}
    \label{fig:gpt2_precision_recall}
    }
    \subfigure[Privacy Audit of an MLP on the Adult dataset.]{\includegraphics[width=0.23\textwidth]{images/tab_precision_recall_full3.pdf}
    \label{fig:image3}
    }


  \caption{Comparison of precision vs recall between \acronym and the baseline $b$}
  \mishaal{we should be consistent in the table and plots for the order of models' epochs; should it be increasing or decreasing order? In the tables it's currently increasing order, let's keep that for everywhere?}
  \label{fig:comparison_precision}
\end{figure*}



%%%ALI: This is the old version with minipage, which we couldn't refer to subfigures.
% \begin{figure*}[h]

%   \centering
  
%   \begin{minipage}[b]{0.23\linewidth}
   
%     \centering
%     \subfigure[Privacy Audit of Wide ResNet-28-2 on CIFAR10.]{\includegraphics[width=\textwidth]{images/final_CIFAR10_WideResNetwTHEORY_precsion_Recall Curves.pdf}}
%     \label{fig:image2}
  
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[b]{0.23\linewidth}
%     \centering
%     \subfigure[Privacy Audit of a Multi-Label CNN on the CelebA dataset.]{\includegraphics[width=\textwidth]{images/AvfCELEB_precsion_Recall-Curves.pdf}}
%     \label{fig:image3}
%   \end{minipage}
% \hfill
% \begin{minipage}[b]{0.23\linewidth}
 
%     \centering
%     \subfigure[Privacy Audit of the GPT-2 on WikiText-2]{\includegraphics[width=\textwidth]{images/nlp_precision_recall.pdf}}
%     \label{fig:image1}
    
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[b]{0.23\linewidth}
%     \centering
%     \subfigure[Privacy Audit of a Multi-Layer Perceptron on the Adult dataset.]{\includegraphics[width=\textwidth]{images/tab_precision_recall.pdf}}
%     \label{fig:image3}
%   \end{minipage}
%   \caption{Comparison of precision vs recall between \acronym and the baseline $b$}
%   \label{fig:comparison_precision}

% \end{figure*}



\begin{figure*}[h]
    \centering
  
    \subfigure[Empirical Privacy of ResNet101 on CIFAR10]
    {
    \includegraphics[width=0.23\textwidth]{ICML24/images/o1_icml-resnet101-alldata-1-1-2.png} 
        \label{fig:image3}
        }
    \subfigure[Empirical Privacy of Multi-Label CNN on the CelebA]
    {
    \includegraphics[width=0.23\textwidth]{ICML24/images/o1_icml-alldata-celebA3_1.jpg} \label{fig:image3}
        }
   \subfigure[Empirical Privacy of GPT-2 model on WikiText-2]
    {
    \includegraphics[width=0.23\textwidth]{ICML24/images/nlp_RMFN_privacy_recall.pdf} \label{fig:gpt2_privacy_recall}
        }
\subfigure[Empirical Privacy of an MLP on the Adult dataset.]{\includegraphics[width=0.23\textwidth]{images/tab_privacy_recall_full3.pdf}\label{fig:image2}}
    
    \caption{Comparison of $\{c+\epsilon\}_{lb} $ vs recall on different datasets.}
    \label{fig:comparison}
\end{figure*}


%%%ALI: This is the old version with minipage, which we couldn't refer to subfigures.

% \begin{figure*}[h]
%   \centering
%    \begin{minipage}[b]{0.24\linewidth}
%     \centering
%     \subfigure[Empirical Privacy of Wide-ResNet-28-2 on CIFAR10]{\includegraphics[width=\textwidth]{images/n_epsilon-glines_wide_resnetfinal.pdf}}
%     \label{fig:image3}
%   \end{minipage}
%   \hfill
%      \begin{minipage}[b]{0.24\linewidth}
%     \centering
%     \subfigure[Empirical Privacy of Multi-Label CNN on the CelebA]{\includegraphics[width=\textwidth]{images/acelebverified_epsilon-glines-1.png}}
%     \label{fig:image3}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.24\linewidth}
 
%     \centering
%     \subfigure[Empirical Privacy of GPT-2 model on WikiText-2]{\includegraphics[width=\textwidth]{images/nlp_privacy_recall.pdf}}
%     \label{fig:gpt2_privacy_recall}
    
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[b]{0.24\linewidth}
   
%     \centering
%     \subfigure[Empirical Privacy of a Multi-Layer Perceptron on the Adult dataset.]{\includegraphics[width=\textwidth]{images/tab_privacy_recall.pdf}}
%     \label{fig:image2}
  
%   \end{minipage}%
  
 

%   \caption{Comparison of $\{c+\epsilon\}_{lb} $ vs recall on different datasets.}
%   \label{fig:comparison}

% \end{figure*}


\begin{figure*}[t]
  \centering

    \subfigure[Number of predictions of ResNet101 on CIFAR10]{\includegraphics[width=0.23\textwidth]{ICML24/images/101ResNet_Predictions.pdf}
    \label{fig:image3}
    }
    \subfigure[Number of predictions of Multi-Label CNN on the CelebA]{\includegraphics[width=0.23\textwidth]{ICML24/images/CELEBA_Predictions.pdf}
    \label{fig:image3}
    }
    \subfigure[Number of predictions of GPT-2 model on WikiText-2]{\includegraphics[width=0.23\textwidth]{images/nlp_RMFN_pred_recall.pdf}
    \label{fig:gpt2_numpred_recall}
    }
    \subfigure[Number of predictions of an MLP on the Adult dataset.]{\includegraphics[width=0.23\textwidth]{images/tab_nbpred_recall_full.pdf}
    \label{fig:image2}
    }
    
  \caption{Comparison of the number of true positives and predictions on different datasets}
  \label{fig:elb_comparison}

\end{figure*}


% \begin{figure*}[h]
%   \centering
%    \begin{minipage}[b]{0.24\linewidth}
%     \centering
%     \subfigure[Number of predictions of Wide-ResNet-28-2 on CIFAR10]{\includegraphics[width=\textwidth]{images/WideResNet_Predictions-.pdf}}
%     \label{fig:image3}
%   \end{minipage}
%   \hfill
%      \begin{minipage}[b]{0.24\linewidth}
%     \centering
%     \subfigure[Number of predictions of Multi-Label CNN on the CelebA]{\includegraphics[width=\textwidth]{images/CELEBA_Predictions-Dataset Size.pdf}}
%     \label{fig:image3}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.24\linewidth}
 
%     \centering
%     \subfigure[Number of predictions of GPT-2 model on WikiText-2]{\includegraphics[width=\textwidth]{images/nlp_pred_recall.pdf}}
%     \label{fig:elb-gpt2}
    
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[b]{0.24\linewidth}
   
%     \centering
%     \subfigure[Number of predictions of a Multi-Layer Perceptron on the Adult dataset.]{\includegraphics[width=\textwidth]{images/tab_nbpred_recall.pdf}}
%     \label{fig:image2}
  
%   \end{minipage}%
  
 

%   \caption{Comparison of the number of true positives and predictions on different datasets}
%   \label{fig:elb_comparison}

% \end{figure*}

% \begin{figure*}[h]


%   \centering
%   \begin{minipage}[b]{0.3\linewidth}
 
%     \centering
%     \subfigure[Privacy Audit of a MLP on the adult dataset]{\includegraphics[width=\textwidth]{images/tab_precision_recall.pdf}}
%     \caption{Precision recall curve obtained from our audit scheme on Adult dataset. Dashed line represent the theoretical maximum precision value given $c_\textrm{lb}= 1.75$, $({c+\epsilon})_{\textrm{lb}} MLP 10 epochs= 2.20$ and $$({c+\epsilon})_{\textrm{lb}} MLP 100 epochs= 3.09$
    
%     }
%     \label{fig:image1}
    
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[b]{0.3\linewidth}
   
%     \centering
%     \subfigure[Empirical privacy of a MLP on Adult dataset]{\includegraphics[width=\textwidth]{images/tab_privacy_recall.pdf}}
%     \caption{Caption for the second image}
%     \label{fig:image2}
  
%   \end{minipage}%
%   \hfill
%   \begin{minipage}[b]{0.3\linewidth}
%     \centering
%     \subfigure[Privacy Audit of a MLP on the adult dataset]{\includegraphics[width=\textwidth]{images/tab_nbpred_recall.pdf}}
%     \caption{Caption for the third image}
%     \label{fig:image3}
%   \end{minipage}

%   \caption{Comparison of privacy audits on different datasets}
%   \label{fig:comparison}

% \end{figure*}



%\vspace{-0.07\baselineskip}
%We assess the effectiveness of our privacy auditing mechanism by running \acronym on ResNet101 and Wide ResNet-28-2 target models \model trained to varying numbers of training epochs; Each of these target models \model are trained on the CIFAR10 dataset comprising 10,000 images, trained to a maximum of 88\% validation accuracy on this dataset size for the ResNet101 and 80\% for the Wide ResNet in the non-overfit case. Also included in our assessment is a Multi-Label CNN classifying 40 attributes associated with each image of the CelebA dataset of 128x128 resolution. The generalized model achieves a test accuracy of 89\% after training on approximately 1,055,000 images (half the actual CelebA dataset). Our MIA has black-box access to the target model, well suited to practical applications, with its input as raw member and non-member (synthetic) data along with loss values of the target model on these member and non-member data points. 
%\ali{this part might need to be moved to the baseline section in V. Also, the point about fairness is not relevant anymore I think. }For fairness in comparison, we provide our baseline classifier $C$ with the loss values of another model $g$, in this case, a ResNet101 trained to the same test accuracy as our target ResNet101 i.e. 88\% on a dataset with the same distribution as the train set of \model, but not a subset of the member data used to train \model. That is:
%$D_f \subseteq \mathcal{D}, \quad D_{\text{out}} \subseteq \mathcal{D}, \quad D_g \subseteq \mathcal{D} \text{ and }D_f \cap D_{\text{out}} = \emptyset, \quad D_f \cap D_g = \emptyset, \quad D_{\text{out}} \cap D_g = \emptyset, \text{ and } D_{\text{in}} \subseteq D_f$.

%The over-fit model epochs are chosen based on a threshold of validation loss peaks vs. train loss, whilst achieving a reasonable test accuracy, as well as loss separability of member and non-member data points in the overfit case, as shown in figure \ref{fig:losses}.

%{\bf Results.} The results, as  shown in \ref{fig:overfitting_comparison}, follow the intuitive expectation that an overfit model memorizes more training data as compared to a generalized one, hence our MIA performs better at low FPRs for a more overfit model \model. In general, however, our technique does better than the baseline classifier in overfit as well as the generalized case for both the CIFAR10 and CelebA datasets. We prove the effectiveness of our technique with the adversary trained on only $N=$ 3000 datapoints (with $N/2=$ member datapoints and $N/2=$  synthetic non-member datapoints), well-suited in federated learning scenarios with limited data available with each client. 



%%%%%%%%%%%




\subsection{General Auditing Results}
\label{subsec:general-results}

Recall that \acronym relies on the quality of synthetic data to measure privacy loss. This quality is assessed by the baseline, from which we can compute $\clb$, a lower bound on $c$-closeness for $\gG$.
%
Focusing on the blue line for the baseline, Figure~\ref{fig:comparison_precision} shows the precision-recall curve for the task of membership inference (looking only at raw data for the baseline) \hadrien{I think raw data + embedding}.
For each value of recall on the x-axis, the precision achieved by the baseline coupled with Proposition \ref{prop:gen-test} and Corollary \ref{result:confidence-interval} gives a lower bound for $c$, shown in Figure~\ref{fig:comparison}.
Figure \ref{fig:elb_comparison} decomposes the precision in numbers of true positives and the number of predictions for a direct mapping to the propositions. Following lines \ref{algo:max-t-start}-\ref{algo:max-t-end} in the last section of Algorithm \ref{algo:panoramia} and the associated discussion in \S\ref{sec:theory}, we pick the largest lower-bound implied at any recall, $\clb$, shown as the dashed blue line on Figure~\ref{fig:comparison}. The associated upper bound on precision at a recall is shown with a dashed line in Figure~\ref{fig:comparison_precision}.

Focusing on the Cifar-10 dataset as an example, we can see that for high-confidence (low recall) guesses we also have high precision, indicating that the model can identify some real images without error. 
However, the precision rapidly decreases as recall increases, suggesting that distinguishing between real and synthetic data for many examples is harder. 
We observe a similar behavior on the WikiText-2 dataset as well as on the Adult dataset.
For the image datasets, the initial precision of the baseline starts at around 90\% and slowly declines for higher recalls to around 50\% (random guessing).
Thus except for a few images, the baseline cannot distinguish between real and generated images, which suggests high-quality synthetic data.

Proposition \ref{prop:gen-test} and Corollary \ref{result:confidence-interval} let us quantify this performance as $\clb$ values of $2.508$, $2.01$, $2.80$ and $2.34$ on Cifar-10, CelebA, WikiText-2 and Adult datasets respectively (see Table \ref{table:audit_values}). 
As we can see on each dataset, the value of $\clb$ reaches its maximum value at relatively low recall, which is where the implied upper-bound on precision is in contact with the observed precision in Figure~\ref{fig:comparison_precision}.
As an aside, the implication is that training generators with a few more really high-quality samples could help us significantly reduce $\clb$, strengthening \acronym's audit power.  

Having established the value of $\clb$, we proceed to the second part of the hypothesis testing, using Proposition \ref{prop:dp-test} and Corollary \ref{result:confidence-interval} to measure $\{c+\epsilon\}_\textrm{lb}$.
Figure~\ref{fig:comparison_precision} presents the precision-recall curve of $\acronym$'s MIA for different target models from Table \ref{table_metrics}. 
For both image datasets, we can see that the precision-recall curves obtained by the MIA are above the one from the baseline. In other words, the addition of information from the audited model $f$ leads to better performance when distinguishing between real and synthetic images.
We observe similar behavior on the tabular dataset and WikiText-2 data. 
%except for the GPT-2\_E12 variant which we discuss later. 
%Ali: the above line is not relevant anymore.
%On all plots, we can observe that more training epochs (more overfitting) lead to better precision-recall trade-offs and higher maximum precision values.
Similar to the $c$-closeness, we leverage the obtained precision for a given number of guesses to compute the maximum value of $\cpepslb$, presented in figure \ref{fig:comparison}.
For all datasets, we obtain maximum values of $\cpepslb$ greater than $\clb$. 
%except GPT-2\_E12, 
% Ali: the above line is not relevant anymore.

The value of $\tilde\epsilon$ for each target model is the gap between its corresponding dashed line and the baseline dashed line. 
This allows us to compute values of $\tilde\epsilon$ reported in Table \ref{table:audit_values}.
%\hadrien{add a few sentences to describe this table when finished}
%For all experiments, we notice that more training epochs on the audited model lead to greater values of $\{c+\epsilon\}_\textrm{lb}$ Our experiment is coherent with the intuition that more training epochs lead to more over-fitting which in turn leads to more privacy leakage. 
It is also interesting to note that the maximum value of $\cpepslb$ typically occurs at low recall. 
Even if we do not use the same metric (precision-recall as opposed to TPR at low FPR) this is coherent with the findings from Carlini et al. \cite{carlini2022membership}. We can detect more privacy leakage (higher $\cpepslb$ which leads to higher $\tilde\epsilon$) when making a few very confident guesses about membership rather than trying to maximize the number of members found (recall). Table \ref{table:audit_values} collects the value of $\cpepslb$, as well as $\tilde\epsilon = \cpepslb - \clb$ measured by \acronym. We can see that $\tilde\epsilon$ reaches up to $0.962$ on Cifar-10 (ResNet101\_E100), $1.02$ on CelebA (Multi-Label CNN-E100), $1.28$ on WikiText-2 (GPT-2\_E96), and $1.34$ on Adult (MLP\_E100). 

These are non-negligible values of privacy leakage, even though the true value is likely much higher.

% There are also cases in which \acronym is not able to meaningfully measure privacy loss. \mishaal{it could be just zero, if we verify from O(1) and that there is no privacy leakage to detect}
% \ali{This paragraph doesn't fit well with the new results. Will Edit.} By taking a closer look at the precision-recall curve of both the baseline (blue) and \acronym's MIA for GPT-2\_E23 (orange)  on figure \ref{fig:gpt2_precision_recall}  we notice that the precision-recall curve of the MIA is mostly above the baseline. Moreover, the MIA retains a high degree of precision compared to the baseline whose precision decreases when the recall increases. However, both the baseline and GPT-2\_E23 have similar maximum precision values. As a result, we can see in Figure \ref{fig:gpt2_privacy_recall}  that the maximum value for $\cpepslb$ is close to $\clb$ leading to a small $\tilde \epsilon$ value even if the MIA outperforms the baseline. This is due to our independent selection of recall thresholds, which leads to similar maximum values of $\clb$ and $\cpepslb$.

\mishaal{new NLP results will determine how the storyline of the below para needs to be updated.} \ali{Will edit. It needs to be re-written I think wrt the new results and knowing the O(1) epsilon}
As illustrated in Figure \ref{fig:gpt2_privacy_recall}, there exist instances (such as in GPT-2\_E12) where the $\clb$ is as large or even larger than $\cpepslb$ (i.e. there is no guarantee that $\cpepslb \ge \clb$). This implies that, under certain conditions, the baseline could outperform the membership inference attack in \acronym. We can see three primary reasons for this behavior:  (1) The synthetic data might not be of high enough quality. If there is an evident distinction between real and synthetic samples, the baseline cannot be fooled reducing the power of our audit. (2) The MIA in \acronym is not powerful enough. (3) The target model's privacy leakage is indeed low \ali{mention that this target model indeed has the lowest validation loss} \ali{Also, we should discuss the difference to O(1), and argue that O(1) rely on negative predictions}. For GPT-2\_E92, GPT-2\_E46, and GPT-2\_E23 \ali{GPT-2\_E23 is kinda low-ish, so not sure if it fits in this argument} in Figure \ref{fig:gpt2_privacy_recall}, we can claim that given the target model's leakage level, the synthetic data and the MIA can perform the audit to a non-negligible power. For GPT-2\_12, we need to examine the possible reasons more closely.
%By fixing the model leakage, we can study (to some extent) how much room there is to improve the fake data quality optimally. 
% Figure \ref{fig:losses} presents the loss distribution for real member samples (members of the target model), real non-members, and synthetic (non-member) samples under the target model and the embedding model. 
Focusing on generated data, in the ideal case we would like the synthetic data to behave just like real non-member data on figures \ref{subfig:lossdist-gpt-2E12}. If that were the case, $\cpepslb$ would go up (since the MIA uses this loss to separate members and non-members). Nonetheless, predicting changes in $\clb$ remains challenging, as analogous loss distributions do not guarantee indistinguishability between data points themselves (also, we cannot necessarily predict how the loss distribution changes under the helper model $\helper$ in figure \ref{subfig:lossdist-h}).
Hence, reason (1) low generative data quality, seems to be a factor in the under-performance of \acronym.
%Assuming $\clb$ doesn’t increase, for GPT-2\_E25 and GPT-2\_12, we state that the synthetic samples quality is not optimal to perform an audit. 
Moreover, in the case GPT-2\_12,  we observe that real members and non-members have very similar loss distributions. Hence, factor (2) also seems to be at play, and a stronger MIA that does not rely exclusively on the plot may increase auditing power. Finally, the helper model $\helper$ seems to have a more distinct loss distribution when compared to GPT-2\_12. If the MIA had access to both target and helper models, we'd expect $\cpepslb$ to at least match $\clb$.
% \ali{it’s kind of mentioning future work in the middle of the analysis} 
% \ali{should I mention that so our mia can be not strong enough, so other mia attack are worth trying -> again, future work in the middle of analysis.} 

%Finally, similar to what we did for the baseline, we plot on Figure \ref{fig:comparison_precision} the maximum theoretical precision given the maximum values of $\cpepslb$.

%Table \ref{table:audit_values} reports the obtained audit value. We obtain $\tilde \epsilon$ values ranging from 0.07 to 2.08. We notice that the nlp modality is where we have both the highest and lowest $\tilde \epsilon$ value. 
%% description of figure 3 (Mishaal)

\subsection{Privacy Auditing of ML Models with Varying Degrees of Overfitting}  \label{sect_results_overfitting}
{\bf Methodology.}
Varying the number of training epochs for the target model to induce overfitting is known to be a factor in privacy loss \cite{yeom2018privacy, LIRA}.
As discussed in section \ref{subsec:dp-measurement}, since these different variants of target models share the same dataset and task, \acronym can compare them in terms of privacy leaking.

To verify if $\acronym$ will indeed attribute a higher value of $\tilde \epsilon$ to more overfitted models, we train our target models for varying numbers of training epochs. The final train and test accuracy are reported in Table~\ref{table_metrics}. For GPT-2 (as a target model), we report the train and validation loss as a measure of overfitting in figure \ref{fig:gpt-2-target-overtraining-loss}.
Figure~\ref{fig:gpt_losses} shows how the gap between member data points (\emph{i.e.}, data used to train the target models) and non-member data points (both real as well as generated non-members) increases as the degree of overfitting increases, in terms of loss distributions. We study the distribution of losses since these are the features extracted from the target model $f$ or helper model $\helper$, to pass to \acronym and the baseline classifier, respectively. The fact that the loss distributions of member data become more separable from non-member data for more overfitted models is a sign that the corresponding target model could leak more information about its training data.
%Adopting the definition proposed by~\cite{carlini2019secret}, the term \emph{``overfitting''} corresponds to the moment at which validation loss stops decreasing.
%\vspace{-0.07\baselineskip}
We thus run \acronym on each model, and present the results next.

%Adopting the definition proposed by~\cite{carlini2019secret}, the term \emph{``overfitting''} corresponds to the moment at which validation loss stops decreasing.


{\bf Results.} 
In Figure \ref{fig:comparison_precision}, we observe that more training epochs (more overfitting) lead to better precision-recall trade-offs and higher maximum precision values. Our results are further confirmed by figure \ref{fig:elb_comparison} with \acronym being able to capture the number of member data points better than the baseline $b$.

In table \ref{table:audit_values}, we further demonstrate that our audit output $\tilde\epsilon$ orders the target models in terms of privacy leakage: higher the degree of overfitting, more memorization and hence a higher $\tilde\epsilon$ returned by \acronym. 
From our experiments, we consistently found that as the number of epochs increased, the value of $\tilde\epsilon$ also increased. For instance, in the WikiText-2 dataset, since we observe $\cpepslb^{\text{GPT-2\_E92}} > \cpepslb^{\text{GPT-2\_E46}} > \cpepslb^{\text{GPT-2\_E23}} > \cpepslb^{\text{GPT-2\_E12}}$, we would have $\cpepslb^{\text{GPT-2\_E92}} - \clb > \cpepslb^{\text{GPT-2\_E46}} - \clb > \cpepslb^{\text{GPT-2\_E23}} - \clb > \cpepslb^{\text{GPT-2\_E12}} - \clb$, , which leads to $\tilde\epsilon_{\text{GPT-2\_E92}} > \tilde\epsilon_{\text{GPT-2\_E46}} > \tilde\epsilon_{\text{GPT-2\_E23}} > \tilde\epsilon_{\text{GPT-2\_E12}}$.
\mishaal{equation is hard to read;}
Our experiment is coherent with the intuition that more training epochs lead to more over-fitting, leading to more privacy leakage measured with a higher value of $\tilde \epsilon$.


\subsection{Privacy Auditing of Differentially Private (DP) ML Models}
\label{subsec:eval:dp-target}

\mishaal{ResNet18 results below; WRN-16-4 DP results in the appendix}
 
{\bf Methodology.} 
We evaluate the performance of \acronym on differentially private (DP) ResNet-18 models on the CIFAR10 dataset under different target privacy budgets ($\epsilon$) and the non-private ($\epsilon=\infty$) cases. The models are trained using the DP-SGD algorithm \citep{abadi2016deep} which we tune each one independently for the highest train accuracy. We include more results and discussions in Appendix \ref{appendix:dp_sup_results}.

{\bf Results.} 
Table \ref{tab:dpResNet18-table} shows that at $\epsilon=2$ (a more private model) \acronym suggests no privacy leakage is detected, whereas at higher values of $\epsilon$ (less private models) and $\epsilon=\infty$ (a non-private model) \acronym detects higher $\tilde{\epsilon}$ values, with $\tilde{\epsilon}_{\epsilon=10} < \tilde{\epsilon}_{\epsilon=15} < \tilde{\epsilon}_{\epsilon=\infty}$, suggesting a lower value of $\epsilon$ leads to lower $\tilde \epsilon$. We compare the performance of \acronym with that of privacy auditing with O(1) training runs \citep{steinke2023privacy}. The conclusion between the two methods is comparable, which potentially suggests more leakage with higher $\epsilon$-DP models.

% \mishaal{this claim is not helpful unless the difference is significant; waiting for higher $\epsilon$-DP models to check numbers on those before editing this section.}
% Even if $\acronym$ returns close $\tilde \epsilon$ values for the two DP models, it still respects the expected ordering and we have $\tilde{\epsilon}_{\epsilon =5} < \tilde \epsilon_{\epsilon=10} < \tilde \epsilon_{\epsilon=\inf}$.
% This experiment confirms that $\acronym$ behaves as expected, a lower value of $\epsilon$ leads to lower $\tilde \epsilon$.

% Bridging the gap between $\tilde\epsilon$ and $\epsilon$ is an interesting avenue for future work.
% o1_icml_resNet18-dp-1.png
\begin{table}
    \centering
    \resizebox{0.45\textwidth}{!}{
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        \textbf{Target model} & \textbf{Audit} & $\mathbf{c_{lb}}$ & $\mathbf{\varepsilon + c_{lb}}$ & $\mathbf{\tilde{\varepsilon}}$ & $\mathbf{\varepsilon}$ \\
        \hline
        ResNet18 $\epsilon=\infty$ & \acronym RM;GN & 2.508 & 3.6698 & 1.161 & - \\
                             & O (1) RM;RN & - & - & - & 1.565 \\
        \hline
        ResNet18 $\epsilon=15$& \acronym RM;GN & 2.508 & 3.5707 & 1.062 & - \\
                           & O (1) RM;RN & - & - & - & 1.22 \\
        \hline
        ResNet18 $\epsilon=10$& \acronym RM;GN & 2.508 & 2.8 & 0.3 & - \\
                           & O (1) RM;RN & - & - & - & 0.14 \\
        \hline
        ResNet18 $\epsilon=2$ & \acronym RM;GN & 2.508 & 2.065 & 0 & - \\
                          & O (1) RM;RN & - & - & - & 0.08 \\
        \hline
    \end{tabular}}
    \caption{Privacy audit of ResNet18 under different values of $\epsilon$-Differential Privacy (DP) using \acronym and O(1) auditing frameworks, where $RM$ is for real member, $RN$ for real non-member and $GN$ for generated (synthetic) non-members. }
    \label{tab:dpResNet18-table}
\end{table}


